The HaLLMark Effect: Supporting Provenance and Transparent Use of Large Language Models in Writing with Interactive Visualization

The use of Large Language Models (LLMs) for writing has sparked controversy both among readers and writers. On one hand, writers are concerned that LLMs will deprive them of agency and ownership, and readers are concerned about spending their time on text generated by soulless machines. On the other hand, AI-assistance can improve writing as long as writers can conform to publisher policies, and as long as readers can be assured that a text has been verified by a human. We argue that a system that captures the provenance of interaction with an LLM can help writers retain their agency, conform to policies, and communicate their use of AI to publishers and readers transparently. Thus we propose HaLLMark, a tool for visualizing the writer's interaction with the LLM. We evaluated HaLLMark with 13 creative writers, and found that it helped them retain a sense of control and ownership of the text.

==> scraps.tex <==
\section{Introduction}

Large Language Models (LLMs) are here to stay.
Their arrival has been particularly widely panned in the area of creative writing, where doomsayers are hinting at a future where it will become impossible to distinguish between a writer's original work and text generated by an LLM.
Worse yet, they may cause us to become inundated with a cornucopia of poor text.
What happens to original thought if we are subjected to writing forever recycled and regurgitated from original work that has been already been produced by our forebears?
It has even been argued that some essential aspect of what it means to be human is lost if creative writing is performed by machines.
While these are valid concerns, it remains that LLMs are just another tool in a long line of tools, and we should find ways to harness the technology in a just, responsible, and ethical way rather than attempt to suppress it.
% Just like video did not, in fact, kill the radio star, the question should not be whether or not LLMs should be employed for creative writing, but how they can be utilized as \textit{supertools}~\cite{Shneiderman2022} to help creative writers improve their craft while maintaining their agency, personal voice, and oversight over the content that has been generated.
But in trying to embrace this technology, one critical concern for writers who want to use LLMs is properly attributing contributions from the AI.
This gives rise to ``ownership tension'' among writers and hampers writer's agency and control over the process~\cite{DBLP:conf/ACMdis/GeroLC22, DBLP:conf/chi/MirowskiMPE23}.
Identifying contributions from AI is also important for writers who need to conform to AI-assisted writing policy~\cite{copyright, authors_guild}.
Publishers have started to articulate rules in these policies, but authors have few tools to track their accountability with regard to these rules and policies. 
% While state-of-the-art LLMs are certainly capable of one-shot generation of an entire narrative in response to a prompt, professional writers tend to want to use LLMs to become \textit{better} writers, not \textit{faster} ones.
% Therefore, the true measure of quality is the \textbf{degree of involvement} between the writer and the LLM~\cite{lee2022coauthor}. \fanny{Here more explicitly mention the concerns around ``intellectual ownership'' -- people want to be recognized for their creative skills (even if they received external aids for inspiration or style polish); and readers want to know a human was behind the writing.}
% \fanny{Second point is -- getting help is ok, so long as this falls within the rules. Publishers started to articulate rules, but authors have few tools to track their accountability with regard to these rules and policies.}
% After all, people tend to favor specialty products---jewelry, pottery, traditional clothing, and artisanal food---when they are handcrafted by artisans rather than manufactured by machines because of authenticity, attention to detail, and artistic expression. 
% However, just as the cheesemaker has his press, the vigneron his fermenter, and the milliner his sewing machine, presumably the writer's tools could be said to include LLMs as long as the writer's influence on the final writing is clear.
% Put differently, only by disclosing the provenance of input from both human and LLMs can we elevate human effort as the gold standard for creative writing. 
% This means that mixed-interaction tools that faithfully capture the provenance of interaction between both humans and LLMs will become central to such novel co-writing workflows.

In this work, we argue that capturing interactions between AI and writers and supporting interactive provenance of those interactions may improve the writer's agency, control, and ownership of the final artifact (e.g., fiction, poems).
Prior research suggests provenance often helps balance automation and agency in human-AI collaboration~\cite{Shneiderman2022}.
Interaction history can also help writers conform to AI-assisted writing policies and be transparent to publishers and readers.
To explore this design space, we first reviewed existing guidelines and policy documents on the use of LLMs from several professional, educational, and academic organizations (Section~\ref{sec:formative}).
The review informed us about the types of information that writer's should be aware of in AI-assisted writing.
We then developed \textsc{\toolname}, a web-based design probe that integrates an authoring interface with LLM support, and stores and visualizes writer's interaction with an LLM.
The system facilitates writers to self-reflect on their use of AI by clearly highlighting contribution from AI.

% In this paper, we present \textsc{\toolname}, a web-based mixed interaction system that integrates an LLM with an authoring interface that combines prompting, original writing, and editing with an interactive graph representation that we call the ``document X-ray.''
% The  authoring interface provides a streamlined interface for generating new content through both free-form prompts as well as several standardized creative composition interactions, such as ``summarize,'' ``elaborate,'' ``enumerate,'' ``introduce,'' and ``conclude.''
% \toolname{} leverages interactive visualization to represent the provenance of text in a document generated by both human authors and LLMs.
% The document X-ray shows the provenance of how each character, word, and sentence was created: either through original writing, a prompt, or a combination of both.
% These operations are also captured in an event visualization that shows how the document has changed over time. 

% We designed \toolname{} based on an extensive literature survey and requirement analysis performed on guidelines and policy documents on the use of LLMs from several professional, educational, and academic organizations (Section~\ref{sec:related-work}). 
% We used these findings to derive a set of design requirements for mixed-initiative co-writing for humans and LLMs (Section~\ref{sec:requirement}).
% We then designed and implemented \toolname{} using modern web technologies (Section~\ref{sec:system}).

To validate \toolname{}, we engaged a group of professional creative writers to use it to write a short story during remote evaluation sessions and collected their feedback and resulting story (Section~\ref{sec:eval}).
Our findings suggest \toolname{} encouraged writers to actively evaluate AI-assistance from the beginning of the writing.
As a result, it instilled a sense of control in writer's mind and improved ownership of the final artifact.
Our findings also suggest \toolname{} will help writers conform to AI-assisted writing policies without the need for manually generating disclosures.
As a result, writers were confident that \toolname{} will help them become more transparent and the tool is an effective medium to communicate the use of AI in producing the artifact to others (i.e., publishers).
We close the paper by outlining the broader impact of our work  on ethical use of LLMs in writing and publication industry (Section~\ref{sec:disc}).

